Spin Correlations in Dark Photon Searches

We investigate the spin correlations between production and decay in the process where dark photons $A'$ are produced in pseudoscalar meson decays, for example, $\pi^0, \eta \to \gamma A'$, and then decay to fermion pairs, $A' \to f \bar{f}$. This process is the focus of many experimental searches, but spin correlations are typically ignored. We derive analytic results that allow us to quickly scan parameter space and quantify the error made in neglecting spin correlations. In particular, we define a discrepancy parameter and find that this parameter is always less than $\frac{1}{6\sqrt{3}} \approx 9.6\%$, which provides a rough measure of the size of spin correlation effects. However, these effects may be enhanced or suppressed by cuts in realistic experimental analyses, and so we also consider two representative examples, including current FASER analyses and possible future searches at SHiP. We find that the effects of spin correlations are negligible for existing FASER analyses, but can significantly reduce event rates at upcoming SHiP searches.

==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}
%\usepackage{caption}
%\usepackage{subcaption}
\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{svg}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{pifont}
\usepackage{subcaption}

\usepackage{lipsum}
\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}
% Boldface vectors, differential del, tikz-feyn, mathrm differentials and probability density
\newcommand{\arccosh}{\mathrm{arccosh}}
\newcommand{\pdensity}{\rho}
\newcommand{\pdensityEnergy}{\rho}
%\newcommand{\de}{\mathrm{d}}
\newcommand{\de}{d}
\renewcommand{\vec}[1]{\mathbf{#1}}
\renewcommand{\Dot}[2]{\left(#1\cdot#2\right)}
\newcommand{\del}{\partial}
\usepackage[compat=1.1.0]{tikz-feynman}
\usepackage{braket}
\usepackage{tensor}
% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\s}{\text{s}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}

\newcommand{\fasernu}{FASER$\nu$~}

\newcommand{\Eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{eq:#1}) and (\ref{eq:#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Secsref}[2]{Sections~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\figssref}[3]{Figs.~\ref{fig:#1}, \ref{fig:#2} and \ref{fig:#3}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}


%comments
\usepackage{xcolor}
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}
%\newcommand{\changed}[2]{#2}
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\definecolor{greenST}{RGB}{0,201,87}
\newcommand{\Seb}[1]{\textcolor{greenST}{[ST: #1]}}
\newcommand{\AI}[1]{\textcolor{red}{[AI: #1]}}
\newcommand{\jlf}[1]{\textcolor{blue}{[JLF: {#1}]}}
\newcommand{\JA}[1]{\textcolor{orange}{[JA: {#1}]}}
\newcommand{\mt}[1]{\textcolor{violet}{[MT: {#1}]}}
\newcommand{\done}[1]{\textcolor{teal}{[JLF: {#1}]}}
\newcommand{\mtoman}[1]{\textcolor{magenta}{[MT: {#1}]}}
\newcommand{\ewelch}[1]{\textcolor{teal}{[EW: {#1}]}}
\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}

%Scintillator cut styling
% \newcommand{\scinton}{\fcolorbox{black}{green}{\rule{0pt}{4pt}\rule{4pt}{0pt}}}
% \newcommand{\scintoff}{\fcolorbox{black}{red}{\rule{0pt}{4pt}\rule{4pt}{0pt}}}
% \newcommand{\scintagn}{\fcolorbox{black}{gray}{\rule{0pt}{4pt}\rule{4pt}{0pt}}}
\newcommand{\scinton}{\text{\cmark}}
\newcommand{\scintoff}{\text{\xmark}}
%\newcommand{\scintagn}{\fcolorbox{black}{gray}{\rule{0pt}{4pt}\rule{4pt}{0pt}}}
\newcommand{\scintagn}{-}

%Ref Style
\bibliographystyle{utphys}

